Emotional Theory of Mind: Bridging Fast Visual Processing with Slow Linguistic Reasoning

The emotional theory of mind problem requires facial expressions, body pose, contextual information and implicit commonsense knowledge to reason about the person's emotion and its causes, making it currently one of the most difficult problems in affective computing. In this work, we propose multiple methods to incorporate the emotional reasoning capabilities by constructing "narrative captions" relevant to emotion perception, that includes contextual and physical signal descriptors that focuses on "Who", "What", "Where" and "How" questions related to the image and emotions of the individual. We propose two distinct ways to construct these captions using zero-shot classifiers (CLIP) and fine-tuning visual-language models (LLaVA) over human generated descriptors. We further utilize these captions to guide the reasoning of language (GPT-4) and vision-language models (LLaVa, GPT-Vision). We evaluate the use of the resulting models in an image-to-language-to-emotion task. Our experiments showed that combining the "Fast" narrative descriptors and "Slow" reasoning of language models is a promising way to achieve emotional theory of mind.

==> Sections/dataset.tex <==
We use the EMOTIC dataset which covers 26 different labels as shown in Table \ref{table-baselines}. The related emotion recognition task is to provide a list of emotion labels that matches those chosen by annotators.
% , responding to the question of, ``How does the person in the bounding box feel?". 
The training set (70\%) was annotated by 1 annotator, where Validation (10\%) and Test (20\%) sets were annotated by 5 and 3 annotators, respectively. 

% The EMOTIC baseline estimation method used a CNN to extract features from the target human, as well as global features over the entire image, and incorporate the two sources using a fusion network~\cite{kosti2019context}. This resulted in a mean average precision (mAP) of 28.33. 


%-----

%\todo{add number of train, test, val}. \todo{add the number of annotators per person for val/train/test}. 
%\yasaman{This is from emotic: After the first round of annotations (1 annotator per image), we divided the images into three sets: Training (70%), Validation (10%), and Testing (20%) maintaining a similar affective category distribution across the different sets. After that, Validation and Testing were annotated by 4 and 2 extra annotators respectively. As a consequence, images in the Validation set are annotated by a total of 5 annotators, while images in the Testing set are annotated by 3 annotators (these numbers can slightly vary for some images since we removed noisy annotations).}


==> Sections/discussion.tex <==
% \begin{itemize}
%     \item howing other people in bb
%     \item missing interactions
%     \item hard to see faces 
% \end{itemize}
% Sympathy does not appear to be well understood by CLIP or GPT-3, often co-occuring with negative emotions (see Table \ref{tab:images}).
% It is possible that breaking down the task into two steps - captioning followed by reasoning - is not the manner in which humans perform the emotional theory of mind task. It is possible that for each emotion, perception is tuned to emotion-specific, salient traits, which could resulting in a different captions for each emotion. This could be an interesting area for future work.
% PAIN
% Painful events are not clearly understood, e.g. childbirth, being hit in a boxing match. 
% FEAR
% peeking out of blinds - but the fine, physical characteristics of being bruised are key
% EMBARASSMENT
% CONFUSION
% SYMPATHY - b3fmbjeeaz873xzcpu_1
% The person in the image is likely experiencing a mix of emotions, including sadness, sympathy, and possibly annoyance or discomfort. The set of six most likely labels that the person is feeling at the same time would be: sadness, sympathy, annoyance, discomfort, disconnection, and possibly fear or embarrassment. These emotions can be inferred from the person's body language, facial expressions, and the context of the image, which shows a woman sitting on a couch with another person offering comfort by placing a hand on her back.
% CAUSAL factors
% Effect of 1-2-more people
%\subsection{Effect of Group Behavior}
Our findings showed that images with a single person resulted in better accuracy than images with two or more people in them (see Table \ref{table:num_people}). One reason for this could be attributed to the lack of social interaction signals in our captions. Images with more than two people had the lowest accuracy results. The literature on group emotions suggests, the shared condition in the group such as the environment and group information could affect the individual emotions within the group \cite{veltmeijer2021automatic}. In our proposed model and linguistic descriptors, contextual information mostly relied on environmental information, with some inclusion of group events (e.g., "black tie event", "party"). For example, Fig.~\ref{tab:fail}.3 shows a possible group of friends, which was not captured by the captioning method. Further, in some cases where the physical signals of the person in the bounding box are not readily available, humans tend to rely on the information from the physical signals from other individuals within the same group to infer and reason about the emotions of a single individual of that group, which is referred as a bottom-up approach \cite{barsade1998group}. In our current proposal, we only use the person in the bounding box's for person descriptors, physical and action signals regardless of its available information content. As an example, the figure in Fig.~\ref{tab:fail}.1 involves multiple individuals in the background that have occluded images with few detectable physical signals, where reasoning about the person's emotions requires to seek meaningful signals from other individuals in the group and the group's behavior as a whole. Our proposed model currently does not allow for these types of emotional reasoning strategies that seems to be an important part of group emotion recognition. % Something about future work here?
% \subsection{Effect of Gender}
% gender -- 
%Our ablation studies showed inclusion of gender signals (e.g., man and woman instead of "an adult") in the generated captions decreased the accuracy of our proposed method (see Table \ref{}). EMOTIC dataset contains 66\% males and 34\% females. The distribution of negative vs. positive labelled emotions in the ground truth were (not) similar between different genders in the images, potentially suggesting a bias in the dataset. Our expectation was to capture this bias with the inclusion of genders in the captions, assuming a similar bias might exists in GPT-3. However, inclusion of gender signals decreased the accuracy. This could result from 1) CLIP not inferring to genders correctly, 2) GPT-3 not having the similar bias as to our ground-truth labels. %Further analysis showed that CLIP was able to infer to the gender of the person in the bounding box \%XX percent of the ... 
% \subsection{Focus on objects in visio-language classifiers}
%Confusing objects in the image to actions.. show the pillow example
Moreover, for the activity and environment detection using CLIP, we performed a standard evaluation with a limited set of classes without a "don't know" or null class, resulting in some mis-captioning. For instance, as shown in Fig.~\ref{tab:fail}.4, the model misunderstood the action as "pillow fight", whereas the action should be described as "covering ears with a pillow", or "yelling". 

% Our inability to pass bounding box in our comparison

==> Sections/humanCaps.tex <==
%\section{Experiments on Human Captions}
\begin{table*}[h!]
\centering
\caption{Performance Metrics for the Small Subset of EMOTIC where human generated captions were available}
\begin{tabular}{
  lcccccc
}
\toprule
{Model} & {Precision (\%)} & {Recall (\%)} & {F1 Score (\%)} & {Hamming Loss (\%)} & {Jaccard Index (\%)} & {Subset Accuracy (\%)} \\
\midrule
NarraCaps + GPT4

HumanCaps + GPT4




\bottomrule
\label{table-baselines}
\end{tabular}
\end{table*}



\mypara{How much improvement can we achieve by enhancing captions?}
\cite{yang2023contextual} recruited an annotator who speaks native North American English. Using a web interface, they manually generated captions for 387 images that contained the 14 negative emotion categories: suffering, annoyance, pain, sadness, anger, aversion, disquietment, doubt/confusion, embarrassment, fear, disapproval, fatigue, disconnection, sensitivity. Negative emotions were the focus of this experiment because they were poorly recognized compared to positive emotions. Initially, using the provided EMOTIC interface\footnote{https://github.com/Tandon-A/emotic/}, we evaluated EMOTIC on these image set and achieved an F1 score of $\textbf{26.50}$ (It is worth mentioning that some of these images are from train and val set). Subsequently, utilizing our narrative captioning method with GPT4, we obtained F1 scores of $\textbf{26.19}$. Conversely, when human-generated captions were input into GPT-4, it resulted in F1 score scores of $\textbf{34.17}$. This suggests that there is a disparity between human-generated captions and our narrative captions, and inspecting the differences to improve the automatic narrative caption method is an interesting area for future work. The result of this experiment suggests promise in using LLMs if the captions can be well defined. It is worth mentioning that, on the same set without the use of intermediate captions, GPT-4 vision, LLaVA, and finetuned LLaVA achieved F1 scores of $\textbf{35.79}$, $\textbf{27.08}$, $\textbf{42.14}$, respectivly.

==> tables/NumberOfPeople.tex <==
% %\begin{table}{r}[width=0.48\textwidth]
% \begin{table}

% \tiny
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{@{}l |ccccccc@{}}
%         \toprule
%          & & CLIP & EMOTIC & NarraCap & GPT4 & LLaVA & LLaVA-f\\
%          \midrule
%         \multirow{3}{2em}{F1}
%         &1 & 16.20 & 32.50 & 26.90 & 34.75 & 20.54 & 23.86\\
%         &2 & 16.67 & 27.60 & 25.81 & 34.28 & 18.97 & 22.85\\
%         &>2 & 16.81 & 24.60 & 24.63 & 32.57 & 18.05 & 16.62\\
%         \midrule
%         \multirow{3}{2em}{SE}
%          &1 & - & - & - & - & - & -\\
%         &2 & - & - & - & - & - & -\\
%         &>2 & - & - & - & - & - & -\\
%         \bottomrule
%         \end{tabular}
%                             }
%     \vspace{-2mm}
%      \caption{Test set mAP and standard error (SE) when separated into 1, 2, and multiple people in the image. Here, NarraCaps is paired with GPT-3.5.}  
     
%       \vspace{-4mm}            
% \label{table:num_people}
% \end{table}




\begin{table}

\tiny
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l |ccccccc@{}}
        \toprule
         & & CLIP & EMOTIC & NarraCap & GPT4 & LLaVA & LLaVA-f\\
         \midrule
        \multirow{3}{2em}{P}
        &1 & 22.07 &  27.72 & 26.44 & 37.53 & 32.06 & 41.27\\
        
        &2 & 21.52 & 23.36 & 26.06 & 36.64 & 36.10 & 38.07\\
        
        &$>$2 & 20.97 & 22.71 & 23.18 & 34.31 & 31.30 & 35.02\\
        \midrule
        \multirow{3}{2em}{R}
         &1 & 28.76 & 41.62 & 32.94 & 39.07 & 22.79 & 41.41\\
         
        &2 & 28.11 & 35.09 & 35.02 & 38.67 &  22.15 & 41.21\\
        &$>$2 & 27.45 & 28.51 & 31.74 & 36.54 & 18.39 & 35.66\\
        \midrule
        \multirow{3}{2em}{F1}
        &1 & 16.20 & 32.50 & 26.53 & 34.75 & 23.53 & 38.42\\
        
        &2 & 16.67 & 27.60 & 27.61 & 34.28 & 23.38 & 37.35\\
        &$>$2 & 16.81 & 24.60 & 25.01 & 32.57 & 19.77 & 33.34\\
        \bottomrule
        \end{tabular}
                            }
    %\vspace{-2mm}
     \caption{Test set precision(p), recall(r), and F1 score when separated into 1, 2, and multiple people in the image. Here, NarraCaps is paired with GPT-4}  
     
      %\vspace{-4mm}            
\label{table:num_people}
\end{table}


==> tables/NumberOfPeople_v0.tex <==
% %\begin{table}{r}[width=0.48\textwidth]
% \begin{table}[!t]
% \small
%     \caption{Test set mAP and standard error (SE) when separated into 1, 2, and multiple people in the image.}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{@{}l |ccccc@{}}
%         \toprule
%          & & NarraCaps & LLaVA & CLIP & ExpNet\\
%          \midrule
%         \multirow{3}{2em}{mAP}

%         &1 & 19.18 & 18.66 & 18.61 & 19.50 \\
%         &2 & 18.66 & 18.61 & 18.28 & 18.40 \\
%         &>2 & 17.88 & 17.85 & 17.78 & 17.76\\
%         \midrule
%         \multirow{3}{2em}{SE}
%          &1 & 0.18 & 0.16 & 0.14 & 0.17 \\
%         &2 & 0.17 & 0.16 & 0.15 & 0.15 \\
%         &>2 & 0.15 & 0.14 & 0.14 & 0.14\\
%         \bottomrule
%         \end{tabular}
%                             }
% \label{table:num_people}
% \end{table}


%\begin{table}{r}[width=0.48\textwidth]
\begin{table}

\tiny
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l |ccccc@{}}
        \toprule
         & & CLIP & LLaVA & ExpNet & NarraCaps\\
         \midrule
        \multirow{3}{2em}{mAP}
        &1 & 18.61 & 18.66 & 19.50 & 19.18 \\
        &2 & 18.28 & 18.61 & 18.40 & 18.66 \\
        &>2 & 17.78 & 17.85 & 17.76 & 17.88 \\
        \midrule
        \multirow{3}{2em}{SE}
         &1 & 0.14 & 0.16 & 0.17 & 0.18 \\
        &2 & 0.15 & 0.16 & 0.15 & 0.17 \\
        &>2 & 0.14 & 0.14 & 0.14 & 0.15 \\
        \bottomrule
        \end{tabular}
                            }
    \vspace{-2mm}
     \caption{Test set mAP and standard error (SE) when separated into 1, 2, and multiple people in the image. Here, NarraCaps is paired with GPT-3.5.}  
     
      \vspace{-4mm}            
\label{table:num_people}
\end{table}


==> tables/SE.tex <==
%\begin{table}{r}[width=0.48\textwidth]
\begin{table}[!t]

    \caption{Standard Error for different methods. Top three numbers are results on the \textbf{test} set, and the rest are on \textbf{val}}
    \tiny
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{@{}l ccc@{}}
        \toprule
         Model & MAP & SE \\
         \midrule
        NarraCaps & 18.58 &	0.094 &  \\
        LLAVA & 18.40 & 0.087 & \\
        Clip & 18.25&0.082  &  \\

        \bottomrule
        \end{tabular}
                            }
\label{table:se}
\end{table}

==> tables/ablation.tex <==
\begin{table}[t]
%\begin{wraptable}{r}{0.48\textwidth}
% \vspace{-15mm}
    \centering
    \resizebox{\linewidth}{!}{

        \begin{tabular}{c c c c c| c c c}
        % \hline
        \toprule
        
        \multicolumn{5}{c}{\textbf{Ablation Settings}}

        & \textbf{F1} & \textbf{diff.} & \textbf{SE}\\

        age & gender & environment & action & physical signals &\\
        % \midrule
        \hline
        \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 29.67 & - & 0.78 \\
        
        - & \checkmark & \checkmark & \checkmark & \checkmark &28.41 & +1.26 & 0.73 \\

        \checkmark & - & \checkmark & \checkmark & \checkmark & 29.25 & +0.42 & 0.78 \\
        
        \checkmark & \checkmark & - & \checkmark & \checkmark &  27.27 & +2.4 & 0.78  \\

        \checkmark & \checkmark & \checkmark & - & \checkmark & 23.67 & +6 & 0.70 \\

        \checkmark & \checkmark & \checkmark & \checkmark & - &   29.47 & +0.2 & 0.85  \\ 
      
     
    \bottomrule
        \end{tabular}
    }
 %   \vspace{-2mm}
        \caption{Ablation study using NarraCaps+GPT4 on 1000 randomly selected images from the validation set. Here, we present F1 scores along with their corresponding standard errors.
}
\label{table:ablation}
%\vspace{-4mm}
\end{table}

==> tables/ablation_v0.tex <==
\begin{table}[t]
%\begin{wraptable}{r}{0.48\textwidth}
% \vspace{-15mm}
    \centering
    \resizebox{\linewidth}{!}{

        \begin{tabular}{c c c c c| c c c}
        % \hline
        \toprule
        
        \multicolumn{5}{c}{\textbf{Ablation Settings}}

        & \textbf{mAP} & \textbf{diff.} & \textbf{SE}\\

        age & gender & environment & action & physical signals &\\
        % \midrule
        \hline
        \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 25.54 & - & 0.27\\
        - & \checkmark & \checkmark & \checkmark & \checkmark & 25.46 & -0.08 & 0.25\\

        \checkmark & - & \checkmark & \checkmark & \checkmark & 25.66 & +0.12 & 0.29\\
        
        \checkmark & \checkmark & - & \checkmark & \checkmark & 25.22 & -0.32 & 0.26\\

        \checkmark & \checkmark & \checkmark & - & \checkmark & 24.91 & -0.63 & 0.24\\

        \checkmark & \checkmark & \checkmark & \checkmark & - & 25.1 & -0.44 & 0.24\\ 
      
     
    \bottomrule
        \end{tabular}
    }
    \vspace{-2mm}
        \caption{Ablation study using NarraCaps+GPT-3.5 on 1000 images randomly selected from the validation set.
}
\label{table:ablation}
\vspace{-4mm}
\end{table}

==> tables/ap_per_category_v0.tex <==
% \begin{table*}[t]
% \centering
% \caption{Performance of different models on EMOTIC. Action, NarraCap, and ExpNet captioning use GPT-3 for inference.}
% \tiny
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% Emotions & EMOTIC & Emoticon & Rand & Maj & Rand(W)& Falcon & MPT & Bichuan & CLIP & Action & LLaVA & ExpNet & NarraCap\\
% \hline
% Affection & 27.85 & 45.23 & 13.27 & 13.41 & 13.58&14.91&14.0&14.32 & 22.63 & 18.13 & 22.97 &18.51& 19.61 \\
% \hline
% Anger & 09.49 & 15.46 & 2.45 & 2.45 & 2.42 &3.32&3.14&2.76 & 6.09 & 2.85 & 6.04 &2.87& 5.60 \\
% \hline
% Annoyance & 14.06 & 21.92 & 4.74 & 4.89 & 4.91 &4.89&4.96&5.02& 5.14 & 5.75 & 5.27 &6.42& 6.32 \\
% \hline
% Anticipation & 58.64 & 72.12 & 46.86 & 47.05 & 47.23&47.12&46.87&46.88 & 47.31 & 48.91 & 48.84 &50.18 & 48.59 \\
% \hline
% Aversion & 07.48 & 17.81 & 3.05 & 3.05 & 3.07&3.05&3.08&2.98 & 3.03 & 3.38 & 3.05 & 3.83 & 3.28 \\
% \hline
% Confidence & 78.35 & 68.65 & 47.33 & 47.43 & 47.84&47.61&47.68&47.39 & 52.12 & 51.78& 48.43 & 55.16 & 49.66 \\
% \hline
% Disapproval & 14.97 & 19.82 & 4.61 & 4.55 & 4.54 &4.58&4.43&4.63& 4.44 & 4.77 & 4.63 & 4.93 &4.78 \\
% \hline
% Disconnection & 21.32 & 43.12 & 15.80 & 15.54 & 15.34 &15.46&15.62&15.52& 15.42 & 15.82& 15.52 &17.09& 17.48 \\
% \hline
% Disquietment & 16.89 & 18.73 & 12.45 & 12.43 & 12.25&12.44&12.48&12.60 & 13.40 & 12.70 & 12.45 & 12.86 &13.27 \\
% \hline
% Doubt/Confusion & 29.63 & 35.12 & 14.31 & 14.52 & 14.60&14.51&14.63&14.49 & 14.58 & 14.60 & 14.52 & 14.51 & 15.21 \\
% \hline
% Embarrassment & 03.18 & 14.37 & 1.89 & 1.88 & 1.85&1.89&2.01&1.85 & 1.96 & 2.07 & 2.02 &2.31& 2.03 \\
% \hline
% Engagement & 87.53 & 91.12 & 77.28 & 77.33 & 77.24 &77.42&77.25&77.37& 76.57 & 79.02 & 78.04&79.38 & 78.36 \\
% \hline
% Esteem & 17.73 & 23.62 & 13.33 & 13.64 & 14.03&13.62&13.57&13.63 & 13.75 & 13.81 & 13.64 & 13.67&13.87 \\
% \hline
% Excitement & 77.16 & 83.26 & 47.80 & 47.94 & 47.34&47.90&48.08&47.90 & 48.31 & 53.31 & 54.29 &56.62& 55.06 \\
% \hline
% Fatigue & 09.70 & 16.23 & 6.02 & 5.91 & 5.95 &5.90&6.00&5.93& 7.38 & 6.36 & 6.91 & 7.24 & 6.44 \\
% \hline
% Fear & 14.14 & 23.65 & 3.27 & 3.20 & 3.20 &3.37&3.30&3.28& 3.67 & 3.56 & 4.35 & 4.03 &3.90 \\
% \hline
% Happiness & 58.26 & 74.71 & 48.05 & 47.95 & 48.27 &47.89&48.60&48.44& 52.60 & 48.93 & 53.41 & 49.40 & 52.51 \\
% \hline
% Pain & 08.94 & 13.21 & 2.03 & 1.96 & 1.95 &1.93&1.90&2.02& 1.99 & 2.11 & 2.32 & 2.15 & 2.28 \\
% \hline
% Peace & 21.56 & 34.27 & 14.70 & 14.61 & 14.33 &14.64&14.67&14.71& 16.38 & 16.15 & 15.25 & 16.72 & 16.42 \\
% \hline
% Pleasure & 45.46 & 65.53 & 29.17 & 28.99 & 29.35 &29.11&29.10&29.50& 30.74 & 29.50 & 29.07 &30.30& 31.72 \\
% \hline
% Sadness & 19.66 & 23.41 & 5.32 & 5.34 & 5.40 &5.41&5.87&5.36& 8.20 & 6.22 &8.62&6.97& 8.23 \\
% \hline
% Sensitivity & 09.28 & 8.32 & 2.88 & 2.93 & 2.94 &2.93&2.92&2.92& 3.42 & 2.95 & 2.91 &2.97& 2.93 \\
% \hline
% Suffering & 18.84 & 26.39 & 3.50 & 3.50 & 3.47 &3.60&3.52&4.69& 3.06 & 3.50 & 3.58 &3.50& 3.50 \\
% \hline
% Surprise & 18.81 & 17.37 & 6.34 & 6.14 & 6.15 &6.12&6.16&6.11& 6.87 & 6.11 &6.80& 6.13 &6.11 \\
% \hline
% Sympathy & 14.71 & 34.28 & 8.33 & 8.45 & 8.34 &8.47&8.59&8.30& 9.01 & 8.52 & 8.92& 9.42&9.35 \\
% \hline
% Yearning & 08.34 & 14.29 & 6.48 & 6.47 & 6.45 &6.47&6.42&6.46& 6.40 & 6.58 & 6.46 &6.50& 6.58 \\
% \hline
% \hline
% mAP & 27.38 & 35.48 & 16.97 & 16.98 & 17.00 &17.10&17.11&17.12& 18.25 & 17.98 & 18.40 &18.60& 18.58 \\
% \hline
% \end{tabular}
% }
% \label{table-baselines}
% \end{table*}






% \begin{table*}[t]
% \centering
% \caption{Performance of different models on EMOTIC. Action, NarraCap, and ExpNet captioning use GPT-3 for inference.}
% \tiny
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% Emotions & EMOTIC & Emoticon & Rand & Maj & Rand(W) & CLIP & Action & LLaVA & ExpNet & NarraCap\\
% \hline
% Affection & 27.85 & 45.23 & 13.27 & 13.41 & 13.58 & 22.63 & 18.13 & 22.97 & 18.51 & 19.61 \\
% \hline
% Anger & 09.49 & 15.46 & 2.45 & 2.45 & 2.42 & 6.09 & 2.85 & 6.04 & 2.87 & 5.60 \\
% \hline
% Annoyance & 14.06 & 21.92 & 4.74 & 4.89 & 4.91 & 5.14 & 5.75 & 5.27 & 6.42 & 6.32 \\
% \hline
% Anticipation & 58.64 & 72.12 & 46.86 & 47.05 & 47.23 & 47.31 & 48.91 & 48.84 & 50.18 & 48.59 \\
% \hline
% Aversion & 07.48 & 17.81 & 3.05 & 3.05 & 3.07 & 3.03 & 3.38 & 3.05 & 3.83 & 3.28 \\
% \hline
% Confidence & 78.35 & 68.65 & 47.33 & 47.43 & 47.84 & 52.12 & 51.78 & 48.43 & 55.16 & 49.66 \\
% \hline
% Disapproval & 14.97 & 19.82 & 4.61 & 4.55 & 4.54 & 4.44 & 4.77 & 4.63 & 4.93 & 4.78 \\
% \hline
% Disconnection & 21.32 & 43.12 & 15.80 & 15.54 & 15.34 & 15.42 & 15.82 & 15.52 & 17.09 & 17.48 \\
% \hline
% Disquietment & 16.89 & 18.73 & 12.45 & 12.43 & 12.25 & 13.40 & 12.70 & 12.45 & 12.86 & 13.27 \\
% \hline
% Doubt/Confusion & 29.63 & 35.12 & 14.31 & 14.52 & 14.60 & 14.58 & 14.60 & 14.52 & 14.51 & 15.21 \\
% \hline
% Embarrassment & 03.18 & 14.37 & 1.89 & 1.88 & 1.85 & 1.96 & 2.07 & 2.02 & 2.31 & 2.03 \\
% \hline
% Engagement & 87.53 & 91.12 & 77.28 & 77.33 & 77.24 & 76.57 & 79.02 & 78.04 & 79.38 & 78.36 \\
% \hline
% Esteem & 17.73 & 23.62 & 13.33 & 13.64 & 14.03 & 13.75 & 13.81 & 13.64 & 13.67 & 13.87 \\
% \hline
% Excitement & 77.16 & 83.26 & 47.80 & 47.94 & 47.34 & 48.31 & 53.31 & 54.29 & 56.62 & 55.06 \\
% \hline
% Fatigue & 09.70 & 16.23 & 6.02 & 5.91 & 5.95 & 7.38 & 6.36 & 6.91 & 7.24 & 6.44 \\
% \hline
% Fear & 14.14 & 23.65 & 3.27 & 3.20 & 3.20 & 3.67 & 3.56 & 4.35 & 4.03 & 3.90 \\
% \hline
% Happiness & 58.26 & 74.71 & 48.05 & 47.95 & 48.27 & 52.60 & 48.93 & 53.41 & 49.40 & 52.51 \\
% \hline
% Pain & 08.94 & 13.21 & 2.03 & 1.96 & 1.95 & 1.99 & 2.11 & 2.32 & 2.15 & 2.28 \\
% \hline
% Peace & 21.56 & 34.27 & 14.70 & 14.61 & 14.33 & 16.38 & 16.15 & 15.25 & 16.72 & 16.42 \\
% \hline
% Pleasure & 45.46 & 65.53 & 29.17 & 28.99 & 29.35 & 30.74 & 29.50 & 29.07 & 30.30 & 31.72 \\
% \hline
% Sadness & 19.66 & 23.41 & 5.32 & 5.34 & 5.40 & 8.20 & 6.22 & 8.62 & 6.97 & 8.23 \\
% \hline
% Sensitivity & 09.28 & 8.32 & 2.88 & 2.93 & 2.94 & 3.42 & 2.95 & 2.91 & 2.97 & 2.93 \\
% \hline
% Suffering & 18.84 & 26.39 & 3.50 & 3.50 & 3.47 & 3.06 & 3.50 & 3.58 & 3.50 & 3.50 \\
% \hline
% Surprise & 18.81 & 17.37 & 6.34 & 6.14 & 6.15 & 6.87 & 6.11 & 6.80 & 6.13 & 6.11 \\
% \hline
% Sympathy & 14.71 & 34.28 & 8.33 & 8.45 & 8.34 & 9.01 & 8.52 & 8.92& 9.42&9.35 \\
% \hline
% Yearning & 08.34 & 14.29 & 6.48 & 6.47 & 6.45 & 6.40 & 6.58 & 6.46 &6.50& 6.58 \\
% \hline
% \hline
% mAP & 27.38 & 35.48 & 16.97 & 16.98 & 17.00 & 18.25 & 17.98 & 18.40 &18.60& 18.58 \\
% \hline
% \end{tabular}
% }
% \label{table-baselines}
% \end{table*}




\begin{table*}[t]
% \vspace{-15mm}
\centering
\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Emotions} & \textbf{Rand} & \textbf{Maj} & \textbf{Rand(W)} & \textbf{CLIP} &\textbf{ Action$^{\dagger}$} & \textbf{LLaVA} & \textbf{ExpNet$^{\dagger}$} & \textbf{NarraCap$^{\dagger}$} & \textbf{NarraCap$^{\ddagger}$}\\
\hline
Affection & 13.27 & 13.41 & 13.58 & 22.63 & 18.13 & 22.97 & 18.51 & 19.61 & 20.35\\
\hline
Anger & 2.45 & 2.45 & 2.42 & 6.09 & 2.85 & 6.04  & 2.87 & 5.60 & 5.49\\
\hline
Annoyance & 4.74 & 4.89 & 4.91 & 5.14 & 5.75 & 5.27 & 6.42 & 6.32 & 6.51 \\
\hline
Anticipation & 46.86 & 47.05 & 47.23 & 47.31 & 48.91 & 48.84 & 50.18 & 48.59 & 47.96 \\
\hline
Aversion & 3.05 & 3.05 & 3.07 & 3.03 & 3.38 & 3.05 & 3.83 & 3.28 & 3.11\\
\hline
Confidence & 47.33 & 47.43 & 47.84 & 52.12 & 51.78 & 48.43 & 55.16 & 49.66 & 50.16\\
\hline
Disapproval & 4.61 & 4.55 & 4.54 & 4.44 & 4.77 & 4.63 & 4.93 & 4.78 & 6.14\\
\hline
Disconnection & 15.80 & 15.54 & 15.34 & 15.42 & 15.82 & 15.52 & 17.09 & 17.48 & 16.84\\
\hline
Disquietment & 12.45 & 12.43 & 12.25 & 13.40 & 12.70 & 12.45 & 12.86 & 13.27 & 13.21\\
\hline
Doubt/Confusion & 14.31 & 14.52 & 14.60 & 14.58 & 14.60 & 14.52 & 14.51 & 15.21 & 15.60\\
\hline
Embarrassment & 1.89 & 1.88 & 1.85 & 1.96 & 2.07 & 2.02 & 2.31 & 2.03 & 1.95\\
\hline
Engagement & 77.28 & 77.33 & 77.24 & 76.57 & 79.02 & 78.04 & 79.38 & 78.36 & 78.24\\
\hline
Esteem & 13.33 & 13.64 & 14.03 & 13.75 & 13.81 & 13.64 & 13.67 & 13.87 & 14.10\\
\hline
Excitement & 47.80 & 47.94 & 47.34 & 48.31 & 53.31 & 54.29 & 56.62 & 55.06 & 54.96\\
\hline
Fatigue & 6.02 & 5.91 & 5.95 & 7.38 & 6.36 & 6.91 & 7.24 & 6.44 & 7.04 \\
\hline
Fear & 3.27 & 3.20 & 3.20 & 3.67 & 3.56 & 4.35 & 4.03 & 3.90 & 5.07\\
\hline
Happiness & 48.05 & 47.95 & 48.27 & 52.60 & 48.93 & 53.41 & 49.40 & 52.51 & 53.06\\
\hline
Pain & 2.03 & 1.96 & 1.95 & 1.99 & 2.11 & 2.32 & 2.15 & 2.28 & 2.42\\
\hline
Peace & 14.70 & 14.61 & 14.33 & 16.38 & 16.15 & 15.25 & 16.72 & 16.42 & 16.19\\
\hline
Pleasure & 29.17 & 28.99 & 29.35 & 30.74 & 29.50 & 29.07 & 30.30 & 31.72 & 30.74\\
\hline
Sadness & 5.32 & 5.34 & 5.40 & 8.20 & 6.22 & 8.62 & 6.97 & 8.23 & 13.53\\
\hline
Sensitivity & 2.88 & 2.93 & 2.94 & 3.42 & 2.95 & 2.91 & 2.97 & 2.93 & 3.28\\
\hline
Suffering & 3.50 & 3.50 & 3.47 & 3.06 & 3.50 & 3.58 & 3.50 & 3.50 & 11.26\\
\hline
Surprise & 6.34 & 6.14 & 6.15 & 6.87 & 6.11 & 6.80 & 6.13 & 6.11 & 6.26\\
\hline
Sympathy & 8.33 & 8.45 & 8.34 & 9.01 & 8.52 & 8.92 & 9.42 & 9.35 & 9.47\\
\hline
Yearning & 6.48 & 6.47 & 6.45 & 6.40 & 6.58 & 6.46 & 6.50 & 6.58 & 6.64\\
\hline
\hline
mAP & 16.97 & 16.98 & 17.00 & 18.25 & 17.98 & 18.40 & 18.60 & 18.58 & 19.22\\
\hline
\end{tabular}
}
\vspace{-2mm}
\caption{Performance of different models on the EMOTIC test set. Action, ExpNet and NarraCap are captioning methods, where $\dagger$ denotes emotion inference using GPT-3.5, and $\ddagger$ denotes inference using GPT-4.}
\label{table-baselines}
\vspace{-4mm}
\end{table*}


==> tables/captions.tex <==
\begin{figure*}[ht!]
% \vspace{-15mm}
\centering
\includegraphics[width=0.98\linewidth]{imgs/LLaVA_Captions (2).pdf}
%\framebox(500,300){}
%\framebox[\textwidth]{\rule{0pt}{140pt}}
% \vspace{-2mm}
 \caption{Examples of LLaVA captions using COT.}
    \label{tab:images2}
% \vspace{-4mm}
\end{figure*}
% }]


==> tables/def_table.tex <==
\begin{table*}[t]
\centering

\resizebox{\textwidth}{!}{

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}

    % \toprule
    \hline
    % \multirow{Emotions} &
    \multicolumn{1}{|c|}{Emotions} &
      \multicolumn{1}{c|}{Emotic} &
      \multicolumn{1}{c|}{Emoticon} &
      \multicolumn{1}{c|}{Clip(5)} &
      \multicolumn{1}{c|}{Clip(std)} &
      \multicolumn{1}{c|}{Env} &
      \multicolumn{1}{c|}{Rand} &
      \multicolumn{1}{c|}{Rand(W)} &
      \multicolumn{1}{c|}{Maj} &
      \multicolumn{1}{c|}{Ours} 
      \\
      % \midrule
      \hline
    Affection & - & - & - & - & - & -& - & - & -\\
      \hline
    Anger & - & - & - & - & - & -& - & - & -\\
    \hline
    Annoyance & - & - & - & - & - & -& - & - & - \\
    \hline
    Anticipation & - & - & - & - & - & -& - & - & - \\
    \hline
    Aversion & - & - & - & - & - & - & - & - & -\\
    \hline
    Confidence & - & - & - & - & - & - & - & - & -\\
    \hline
    Disapproval & - & - & - & - & - & - & - & - & -\\
    \hline
    Disconnection & - & - & - & - & - & -& - & - & - \\
    \hline
    Disquietment & - & - & - & - & - & - & - & - & -\\
    \hline
    Doubt/Confusion & - & - & - & - & - & -& - & - & - \\
    \hline
    Embarrassment & - & - & - & - & - & - & - & - & -\\
    \hline
    Engagement & - & - & - & - & - & -& - & - & -\\
    \hline
    Esteem & - & - & - & - & - & -& - & - & -\\
    \hline
    Excitement & - & - & - & - & - & - & - & - & -\\
    \hline
    Fatigue & - & - & - & - & - & - & - & - & -\\
    \hline
    Fear & - & - & - & - & - & - & - & - & -\\
    \hline
    Hapiness & - & - & - & - & - & - & - & - & -\\
    \hline
    Pain & - & - & - & - & - & - & - & - & -\\
    \hline
    Peace & - & - & - & - & - & - & - & - & -\\
    \hline
    Pleasure & - & - & - & - & - & - & - & - & -\\
    \hline
    Sadness & - & - & - & - & - & -& - & - & -\\
    \hline
    Sensitivity & - & - & - & - & - & - & - & - & -\\
    \hline
    Suffering & - & - & - & - & - & -& - & - & -\\
    \hline
    Surprise & - & - & - & - & - & -& - & - & -\\
    \hline
    Sympathy & - & - & - & - & - & -& - & - & -\\
    \hline
    Yearning & - & - & - & - & - & -& - & - & -\\
    \hline
    \hline
    mAP & 
    \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} &
      \multicolumn{1}{c|}{-} \\
    % \bottomrule
    \hline
  \end{tabular}
  }
  \label{table-}
  
\caption{Performance of different models on Emotic dataset.}

\end{table*}

==> tables/emotic_mapping.tex <==
\begin{table*}
\centering
\small
    \caption{The Emotion Thesaurus \cite{puglisi2019emotion} lists physical signals for numerous emotions; we included only the signals from the emotions which were synonyms of the EMOTIC labels listed here.
}
    {
        \begin{tabular}{@{}l l@{}}
        \toprule
        \textbf{EMOTIC Labels} & \textbf{The Emotion Thesaurus} \\
        \midrule
        affection & love, adoration \\
        anger & anger, resentment, rage\\
        annoyance & annoyance, irritation, impatience, frustration\\
        anticipation& anticipation\\
        aversion & disgust, hatred, reluctance  \\
        confidence & confidence, certainty, pride\\
        disapproval & contempt, scorn\\
        disconnection & indifference, boredom\\
        disquietment & nervousness, worry, anxiety\\
        doubt/confusion & confusion, doubt, skepticism\\
        embarrassment & embarrassment, guilt, shame\\
        engagement & curiosity\\
        esteem & gratitude, admiration\\
        excitement & excitement \\
        fatigue & exhaustion, lethargy\\
        fear & fear, suspicious, terror, horror\\
        happiness & happiness, amusement, joy \\
        pain & pain\\
        peace & peacefulness, satisfaction, relaxation\\
        pleasure & pleased\\
        sadness & sadness, disappointment, disappointed, discouragement\\
        sensitivity & vulnerability\\
        suffering & anguish, depression, stress, hurt\\
        surprise & surprise/shock\\
        sympathy & sympathy\\
        yearning & envy, jealousy, desire, lust\\
     
        \bottomrule
        \end{tabular}
    }
\label{table:emotic_mapping}
\end{table*}
%\end{wraptable}

==> tables/env.tex <==



\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{    
    \begin{tabular}{cccc}
        \hline
        \multicolumn{4}{c}{\textbf{Environments}} \\
        \hline
        Alley & Bank & Big City Street & Board Room \\
        Car Accident & Car Wash & Cheap Motel & Community Center \\
        Condemned Apartment Building & Construction Site & Courtroom & Elevator \\
        Emergency Room & Empty Lot & Factory & Fire Station \\
        Fitness Center & Funeral Home & Gas Station & Hair Salon \\
        Homeless Shelter & Hospital Room & Hotel Room & Juvenile Detention Center \\
        Laundromat & Library & Mechanics Shop & Military Base \\
        Morgue & Newsroom & Nursing Home & Office Cubicle \\
        Park & Parking Garage & Parking Lot & Penthouse Suite \\
        Police Station & Prison Cell & Psychiatric Ward & Public Restroom \\
        Refugee Camp & Run-Down Apartment & Sewers & Small Town Street \\
        Spa & Tattoo Parlor & Therapist Office & Underpass \\
        Vet Clinic & Waiting Room & Bakery & Bar \\
        Casual Dining Restaurant & Coffeehouse & Deli & Diner \\
        Fast Food Restaurant & Ice Cream Parlor & Pub & Antiques Shop \\
        Bazaar & Bookstore & Convenience Store & Flower Shop \\
        Grocery Store & Hardware Store & Jewelry Store & Liquor Store \\
        Pawn Shop & Pet Store & Psychics Shop & Shopping Mall \\
        Thrift Store & Used Car Dealership & Amusement Park & Art Gallery \\
        Art Studio & Ballroom & Black-Tie Event & Bowling Alley \\
        Carnival Funhouse & Casino & Circus & Golf Course \\
        Green Room & Indoor Shooting Range & Movie Theater & Museum \\
        Nightclub & Outdoor Pool & Outdoor Skating Rink & Parade \\
        Performing Arts Theater & Pool Hall & Race Track (Horses) & Rec Center \\
        Recording Studio & Rock Concert & Skate Park & Ski Resort \\
        Sporting Event Stands & Vegas Stage Show & Water Park & Zoo \\
        Airplane & Airport & Ambulance & City Bus \\
        Cruise Ship & Fishing Boat & Limousine & Marina \\
        Military Helicopter & Old Pick-Up Truck & Police Car & Submarine \\
        Subway Train & Subway Tunnel & Tank & Taxi \\
        Train Station & Truck Stop & Yacht & Attic \\
        Backyard & Basement & Bathroom & Birthday Party \\
        Block Party & Bomb Shelter & Chicken Coop & Child's Bedroom \\
        Flower Garden & Garage & Greenhouse & Group Foster Home \\
        Halloween Party & House Fire & House Party & Kitchen \\
        Living Room & Man Cave & Mansion & Motor Home \\
        Nursery & Outhouse & Patio Deck & Root Cellar \\
        Secret Passageway & Teenager Bedroom & Toolshed & Trailer Park \\
        Tree House & Underground Storm Shelter & Vegetable Patch & Wake \\
        Wine Cellar & Workshop & Boarding School & Custodial Supply Room \\
        Dorm Room & Elementary School Classroom & Gymnasium & High School Cafeteria \\
        High School Hallway & Locker Room & Playground & Preschool \\
        Principal Office & Prom & School Bus & Science Lab \\
        Teacher Lounge & University Lecture Hall & University Quad & Abandoned Mine \\
        Ancient Ruins & Archery Range & Barn & Beach Party \\
        Campsite & Church & Country Road & County Fair \\
        Farmer Market & Graveyard & Hunting Cabin & Landfill \\
        Lighthouse & Mausoleum & Orchard & Pasture \\
        Quarry & Ranch & Rodeo & Salvage Yard \\
        Slaughterhouse & Summer Camp & Taxidermist & Wedding Reception \\
        Winery & Arctic Tundra & Badlands & Beach \\
        Canyon & Cave & Creek & Desert \\
        Forest & Grotto & Hiking Trail & Hot Springs \\
        Lake & Marsh & Meadow & Moors \\
        Mountains & Ocean & Pond & Rainforest \\
        River & Swamp & Tropical Island & Waterfall \\
        \hline
    \end{tabular}
    }
    \caption{Example listing of environments from \cite{puglisi2016rural, puglisi2016urban}.}
    \label{tab:environments}
\end{table*}




==> tables/fails_copy.tex <==
\begin{table*}[!ht]
\tiny
  \centering
  \caption{Failure examples of the NarraCaps method.}
  \label{tab:fail}
  \begin{tabular}{ccc}
   \includegraphics[width=0.3\textwidth]{imgs/b3fmbjeeaz873xzcpu_1.jpg} &
    \includegraphics[width=0.3\textwidth]{imgs/ddkop7rtr67verjpfd_0.jpg} &
    \includegraphics[width=0.3\textwidth]{imgs/COCO_train2014_000000353009_0.jpg} \\
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{1. GT}: Affection, Doubt/Confusion, Sympathy\\
      \textbf{NarraCap}: This person is an adult who is \wrong{acting in a play} at a therapist office. This person is \wrong{not engaging in conversation.}\\
    \textbf{GPT-3.5}: Aversion, Disapproval, Fear, Annoyance, Disquietment, Embarrassment\\
    \textbf{CLIP}: Disconnection, Disquietment, Esteem, Sensitivity, Anger, Engagement\\
    % \textbf{LLaVA response}:The person in the red bounding box appears to be experiencing a range of emotions, including sadness, sympathy, and possibly fear or concern. They may be feeling sad or empathetic towards the other woman who has her arms folded and is seemingly upset or frustrated. The presence of a couch and remote in the image suggests that they are in a living room, adding to the intimate and personal nature of their interaction. The combination of expressions and body language, along with the presence of a cell phone, indicates that the two women may be engaged in a deep conversation or discussing a difficult topic.\\
    \textbf{LLaVA}: Sadness, Sympathy, Fear\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{2. GT}: Anger, Annoyance, Confidence, Engagement, Excitement, Pain, Suffering\\
      \textbf{NarraCap}: This person is a \wrong{baby} who is punching a person (boxing) at a sporting event stands. This person is \wrong{chewing on a knuckle}. This person is \wrong{propping the head up with fist}. \wrong{This person is responding with anger by punching.}\\
      \textbf{GPT-3.5}: Anger, Fear, Annoyance, Disquietment, Embarrassment, Excitement\\
      \textbf{CLIP}: Suffering, Disapproval, Annoyance, Embarrassment, Sympathy, Anger\\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mix of emotions. The most likely labels they are feeling would include excitement, anticipation, and happiness, as they are engaged in a boxing match and possibly celebrating a victory. They might also be feeling a sense of annoyance or discomfort due to the physical contact with the other boxer. Additionally, they could be experiencing sadness or sympathy for the other boxer, as the fight is competitive, and the emotions of both fighters are likely to be complex. Overall, the range of emotions experienced during a boxing match can vary, and the person in the red bounding box is likely experiencing a combination of these emotions during the fight.\\
      \textbf{LLaVA}: Excitement, Anticipation, Happiness, Annoyance, Sadness, Sympathy\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline 
    \textbf{3. GT}: Anticipation, Confidence, Esteem\\
      \textbf{NarraCap}:
      This person is an \wrong{elderly} person who is doing a tennis swing at a rec center. This person has leg muscles tightening. This person is using the body to nudge, push, or block.\\
      \textbf{GPT-3.5}: Confidence, Engagement, Happiness, Pleasure, Excitement, Anticipation\\
      \textbf{CLIP}: Doubt/Confusion, Esteem, Confidence, Fatigue, Sensitivity, Suffering\\
      % \textbf{LLaVA response}: The person in the red bounding box is likely experiencing a mixture of emotions, including anguish, fear, and sadness, as they are caught in a difficult situation. They may also feel sympathy, as they are seen playing tennis in the black and white photo, possibly with others. The image shows the person is attempting to hit the tennis ball with their racquet, which indicates they are engaged in the game. The fact that the person is in a red box suggests they are the central focus of the scene, and their emotions might be linked to their performance or the outcome of the game.\\
      \textbf{LLaVA}: Fear, Sadness, Sympathy\\
      \hline
    \end{tabular} \\
    \includegraphics[width=0.3\textwidth]{imgs/f36j0deu657obta0ln_0.jpg} &
    \includegraphics[width=0.3\textwidth]{imgs/egnw6lbc92pja8wkok_1.jpg}  &
    \includegraphics[width=0.3\textwidth]{imgs/fn3o5z0u9vxkzs2giz_0.jpg}  \\
    
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{4. GT}: Aversion, Disquietment, Fear, Sadness, Sensitivity, Suffering\\
      \textbf{NarraCap}: This person is an adult who is \wrong{twiddling fingers} at a \wrong{attic}. This person has lips pulling back, baring the teeth. This person has \wrong{skin stretched into a snarl}. This person is \wrong{placing fingertips against one's open mouth}.\\
    \textbf{GPT-3.5}: Fear, Anger, Disapproval, Aversion, Annoyance, Disquietment\\
    \textbf{CLIP}: Sensitivity, Anger, Suffering, Doubt/Confusion, Disconnection, Fear\\
    % \textbf{LLaVA response}: Based on the image, the person in the red bounding box is most likely experiencing a mixture of fear, surprise, and disgust. The hand with long, sharp claws is reaching towards the person's face, which could provoke feelings of unease and threat. The close-up of the face also enhances the sense of immediacy and intensity of the emotions experienced by the person in the box. It is important to note that the image is open to interpretation, and other viewers may perceive different emotions or nuances in the scene \\
      \textbf{LLaVA}: Fear, Surprise \\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{5. GT}: Disapproval, Disquietment, Fear, Sadness, Suffering\\
      \textbf{NarraCap}: This person is an \wrong{elderly} person who is \wrong{huddling} at a \wrong{city bus}. This person is crying, wailing, begging for help. This person is squeezing the eyes shut, refusing to look.\\
      \textbf{GPT-3.5}: Fear, Pain, Anger, Sadness, Embarrassment, Sympathy\\
      \textbf{CLIP}: Engagement, Esteem, Fear, Sensitivity, Sadness, Sympathy \\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mixture of emotions, including sadness, distress, and vulnerability. With the group of people around her, it seems she is seeking comfort or support from others. Her head is covered, which might add to her feelings of distress or sadness. While some of the other people in the scene may also be experiencing hardships, the person in the red bounding box is the main focus, and her emotions are more prominently displayed. It is important to offer help and support to people in such situations to alleviate their pain and assist them in coping with their emotional turmoil\\
      \textbf{LLaVA}: Sadness, Pain \\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{6. GT}: Affection, Anger, Annoyance, Disapproval, Disquietment, Doubt/Confusion, Fear, Sadness\\
      \textbf{NarraCap}: This person is an adult who is having a \wrong{pillow fight} at a run-down apartment. This person is tossing and turning in bed, an inability to sleep.\\
    \textbf{GPT-3.5}: Fear, Annoyance, Fatigue, Embarrassment, Excitement, Sadness\\
    \textbf{CLIP}: Aversion, Sympathy, Sensitivity, Disquietment, Anger, Fatigue\\
    % \textbf{LLaVA response}: Based on the image of the woman with her hands over her face and the visual labels provided, it is likely that she is experiencing a combination of emotions, including sadness, fear, and possibly some confusion or discomfort. The scene might depict feelings of being overwhelmed, anxious or even experiencing a nightmare, given the visual context of the bed and the white pillow. It is important to note that emotions can be complex, and different people may experience different emotions or react differently to the same situation \\
      \textbf{LLaVA}: Sadness, Fear \\
      \hline
    \end{tabular} \\
    \includegraphics[width=0.3\textwidth]{imgs/frame_hgnlox6nq0yw9qbg_1.jpg} &
    \includegraphics[width=0.3\textwidth]{imgs/sun_aiuphnodytonkden_1.jpg}  &
    \includegraphics[width=0.3\textwidth]{imgs/sun_avyraobmgdwerddj_0.jpg}  \\
    
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
        \textbf{7. GT}: Anger, Anticipation, Aversion, Engagement, Excitement, Happiness, Pleasure, Sympathy\\
      \textbf{NarraCap}:  This person is an adult who is longboarding at a skate park. This person has fingers loosely clasped in one's lap. This person has raised, prominent cheekbones from smiling. This person is \wrong{rubbing one's hands on pant legs.}\\
    \textbf{GPT-3.5}: Confidence, Engagement, Happiness, Peace, Pleasure, Esteem\\
    \textbf{CLIP}: Sadness, Surprise, Pain, Esteem, Excitement, Happiness \\
    % \textbf{LLaVA response}: Based on the image, the person in the red bounding box is likely experiencing a mix of emotions. These may include happiness, as they are smiling, as well as a sense of belonging or camaraderie, since they are surrounded by four friends who are also holding skateboards. They might also feel excitement or anticipation, given their engagement in the activity of skateboarding and possibly waiting to perform tricks or enjoy the day ahead. While it is not possible to definitively confirm all six emotions, these are some plausible feelings the person in the red bounding box could be experiencing based on the visual cues provided.\\
      \textbf{LLaVA}: Happiness, Excitement, Anticipation, Engagement\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{8. GT}: Disconnection, Engagement, Peace, Pleasure\\
      \textbf{NarraCap}: This person is a \wrong{baby} who is swinging at a \wrong{tree house}. This person is slouching in a chair \wrong{with one's arms dangling}.\\
      \textbf{GPT-3.5}: Fear, Embarrassment, Annoyance, Fatigue, Disquietment, Sadness\\
      \textbf{CLIP}: Sensitivity, Sympathy, Sadness, Excitement, Pain, Fear\\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mix of emotions. The most likely labels they are feeling would include happiness, as they are on a swing at a park, enjoying the experience. Additionally, some sadness or disappointment may be present since they are described as missing their family and being in pain. The person may also be experiencing anticipation and excitement, as they are looking forward to coming home. Furthermore, the presence of the large purple ball and bench may indicate a sense of curiosity or interest in the surroundings.\\
      \textbf{LLaVA}: Happiness, Sadness, Disappointment, Pain, Anticipation, Excitement\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{9. GT}: Confidence, Disconnection, Engagement, Happiness, Sympathy\\
      \textbf{NarraCap}: This person is an elderly person who is \wrong{conducting an auction} at a \wrong{university lecture hall}. This person is clasping the hands in front of the groin or other sensitive area.\\
    \textbf{GPT-3.5}: Fear, Embarrassment, Disquietment, Annoyance, Doubt/Confusion, Sadness\\
    \textbf{CLIP}: Sympathy, Sensitivity, Esteem, Disapproval, Embarrassment, Surprise\\
    % \textbf{LLaVA response}: Given the image, the person in the red bounding box might be experiencing a mix of emotions. Six possible labels that the person could be feeling include happiness, excitement, anticipation, surprise, admiration, and sympathy. For instance, the person might be happy to attend the meeting, excited about a forthcoming event or discussion, and anticipating a positive outcome. They could also experience surprise at an unexpected development or revelation, feel admiration for a speaker or colleague, and empathize with others' emotions. However, without knowing the specific context, it is difficult to pinpoint the exact emotions the person in the red bounding box is experiencing.\\
      \textbf{LLaVA}: Happiness, Excitement, Anticipation, Surprise, Sympathy\\
      \hline
    \end{tabular} \\
  \end{tabular}
\end{table*}






==> tables/pick_phys_sigs.tex <==
%\begin{table}{r}[width=0.48\textwidth]
\begin{table}[!h]
 \caption{
Results for different approaches of picking physical signals on the $1000$ randomly selected people from validation set. We also report the average number of physical signals and average number of words in captions for each approach.}
\small
   
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}l cccc@{}}
        \toprule
         & mAP & ave \#sigs & ave cap len \\
         \midrule
        top1 & 25.22 & 1.0 & 22.016 &  \\
        top3 & 25.33 & 3.0 & 37.24 & \\
        top5 & 25.35 & 5.0 & 52.506 & \\
        $mean + std$ & 25.43 & 44.512 & 330.15& \\
        $mean + 3\times{std}$ & 25.53 & 12.127 & 104.702 & \\
        $mean + 5\times{std}$ & 25.32 & 5.524 & 56.184 & \\
        $mean + 7\times{std}$ & 25.47 & 3.058 & 37.816 &\\
        $mean + 9\times{std}$ & \textbf{25.54} & \textbf{1.899} & \textbf{28.986} &\\
        \bottomrule
        \end{tabular}
        
                            }
\label{table:pick_sigs}
\end{table}

==> tables/qualitative.tex <==
\begin{table*}[!ht]
\vspace{-15mm}
\tiny
  \centering
  \begin{tabular}{ccc}
    \includegraphics[width=0.3\textwidth]{latex/imgs/frame_5y05qy595o62zq0d_0.jpg} & 
    \includegraphics[width=0.3\textwidth]{latex/imgs/COCO_train2014_000000355562_1.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/frame_4rauu3fxrxpl6t8w_0.jpg} \\
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
          \textbf{1. GT}: Anticipation, Excitement, Happiness, Pleasure, Sympathy\\
      \textbf{NarraCap}: This person is an elderly person who is petting an animal (not a cat) at a nursing home. This person is offering encouragement and support.\\
    \textbf{GPT-3.5}: Confidence, Affection, Engagement, \correct{Happiness}, Peace, Esteem.\\
    \textbf{CLIP}: \wrong{Doubt/Confusion}, Esteem, Sensitivity, Engagement, \correct{Sympathy}, Affection\\
    % \textbf{LLaVA response}:Based on the image, the person in the red bounding box is likely experiencing a mixture of emotions, such as happiness and affection, while interacting with the older woman and her dog. They may also feel a sense of surprise or curiosity as they engage in the interaction, which might involve greeting, shaking hands, or playing with the dog. The person's emotions could be a blend of joy, empathy, and interest while being around the older woman and her pet.\\
    \textbf{LLaVA}: \correct{Happiness}, Affection, Surprise\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
        \textbf{2. GT}: Engagement, Happiness, Peace\\
        \textbf{NarraCap}: This person is an adult who is hugging at a airport. This person is clutching at another person for support. This person is pulling someone into a side hug. This person is putting an arm around someone’s shoulders.\\
       \textbf{GPT-3.5}: Confidence, \correct{Engagement}, \correct{Happiness}, \correct{Peace}, Pleasure, Esteem\\
       \textbf{CLIP}: \wrong{Sensitivity}, \wrong{Disconnection}, \correct{Happiness}, \wrong{Suffering}, \wrong{Surprise}, Affection\\
       \textbf{LLaVA}: \correct{Happiness}, Excitement, \wrong{Sadness}\\
       %"Based on the image, the person in the red bounding box appears to be experiencing a mix of emotions. The most likely labels they are feeling include happiness, as they are smiling, and perhaps excitement, as they are embracing their travel companion. Additionally, they may be experiencing a sense of sadness or nostalgia, as they are seen saying goodbye to their loved ones at the airport. The presence of suitcases and other individuals in the scene further supports the idea that they are in a transitional, emotional state, either departing or arriving from a journey.
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{3. GT}: fatigue, peace\\
      \textbf{NarraCap}: This person is an adult who is sleeping at a library. This person is curling up to take up less space. This person is falling asleep in odd places at odd times.\\
    \textbf{GPT-3.5}: \wrong{Fear}, \correct{Fatigue}, Embarrassment, Disconnection, Sadness, Sympathy\\
    \textbf{CLIP}: Sympathy, \wrong{Engagement}, \wrong{Suffering}, Disquietment, Disconnection, \correct{Fatigue}\\
    % \textbf{LLaVA response}:Based on the visual content, the person in the red bounding box seems to be experiencing a mix of emotions, which may include feelings of being overwhelmed, anxious, or stressed. The image shows a man sleeping while surrounded by a significant number of books, which might suggest that he is a student or someone deeply engrossed in academic work. The combination of sleeping amidst books and the presence of multiple books in close proximity may indicate a challenging situation, where the person is struggling to cope with their workload, or possibly experiencing exhaustion and needing a break. The presence of a clock in the image might also add to the sense of time pressure and urgency the person could be feeling.\\
    \textbf{LLaVA}: - \\
      \hline
      % \vspace{10mm}
    \end{tabular} \\
    
    \includegraphics[width=0.3\textwidth]{latex/imgs/t1-4.png}  &
    % \vspace{-2mm}
    \includegraphics[width=0.3\textwidth]
{latex/imgs/COCO_val2014_000000070426_0.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/COCO_train2014_000000106222_0} \\
    
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{4. GT}: Confidence, Esteem, Excitement, Happiness, Pleasure\\
      \textbf{NarraCap}: This person is an adult who is skiing at a ski resort. This person has hands raised into the air. This person is waving the arms, using grand gestures.\\
    \textbf{GPT-3.5}: \correct{Confidence}, Engagement, \correct{Happiness}, \correct{Pleasure}, \correct{Excitement}, Anticipation\\
    \textbf{CLIP}: \correct{Esteem}, \wrong{Doubt/Confusion}, \wrong{Surprise}, \correct{Happiness}, \correct{Confidence}, \wrong{Fear}\\
    % "The person in the red bounding box is likely experiencing a mix of emotions, including happiness, excitement, and a sense of accomplishment. Standing on skis in the snow with their arms raised, the person appears to be enjoying the outdoor activity and the thrill of skiing down the slope. Simultaneously, they might also feel a sense of sadness or nostalgia as they pose for what might be their last skiing picture of the season. Overall, the person's emotions are a blend of positive feelings related to the activity and a tinge of sentimentality or nostalgia, possibly due to the changing seasons or the end of a skiing adventure."
    \textbf{LLaVA}: \correct{Happiness}, \correct{Excitement}, \wrong{Sadness}\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline


          \textbf{5. GT}: Happiness, Peace, Pleasure\\
      \textbf{NarraCap}: This person is an adult who is surfing water at a beach. This person is participating in relaxing activities.\\
      \textbf{GPT-3.5}: Confidence, Engagement, \correct{Happiness, Peace, Pleasure}, Esteem\\
      \textbf{CLIP}: \correct{Happiness}, \wrong{Sympathy}, \wrong{Embarrassment}, \correct{Peace}, Confidence, Esteem\\
      % \textbf{LLaVA response}: The person in the red bounding box is likely experiencing a mixture of emotions, primarily focused on feelings of happiness, confidence, and excitement, as they are on the beach wearing a bikini and smiling. They may also be feeling a sense of accomplishment or satisfaction, as they are riding a surfboard or boogie board , possibly catching a wave. While the image does not explicitly show signs of pain or anguish, one could infer that the overall positive atmosphere and beach setting contribute to an overall sense of well-being and enjoyment, with the person being engaged and content in the moment.\\
      \textbf{LLaVA}: \correct{Happiness}, Confidence, Excitement, \wrong{Pain}\\
      
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{6. GT}: Anticipation, Confidence, Doubt/Confusion, Engagement, Excitement, Happiness\\
      \textbf{NarraCap}: This person is an adult who is snowboarding at a ski resort. This person has shoulders lowered and loose. This person is pulling arms and legs in toward the core.\\
    \textbf{GPT-3.5}: \correct{Confidence}, \correct{Engagement}, \correct{Happiness}, Pleasure, \correct{Excitement}, \correct{Anticipation}\\
    \textbf{CLIP}: \wrong{Pain}, \wrong{Surprise}, \correct{Doubt/Confusion}, \correct{Confidence}, \wrong{Fear}, \wrong{Suffering}\\
    % \textbf{LLaVA response}: Based on the visual content, the person in the red bounding box appears to be experiencing a mix of emotions. These include sadness, as they seem to be crying, and a sense of being overwhelmed or stuck in a situation. They might also be experiencing fear, as indicated by their body language and the fact that they are on a snowboard. The presence of a backpack suggests that they may be on a longer outdoor adventure or ski trip, which could contribute to their feelings of being tired or worn down. Overall, the set of six most likely labels for the person in the red bounding box would include a combination of sad, overwhelmed, scared, and tired.\\
      \textbf{LLaVA}: \wrong{Fear}, \wrong{Sadness}\\
      \hline
    \end{tabular} \\
    \includegraphics[width=0.3\textwidth]{latex/imgs/e5oq7a3tdo80dbng0n_1.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/35wl8i3o91qva5pmpv_0} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/2chjrlhl4rpx0yaw4l_0.jpg} \\
    
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{7. GT}: Engagement, Sadness, Suffering, Sympathy\\
      \textbf{NarraCap}: This person is an adult who is crying at a refugee camp. This person is crying, wailing, begging for help.\\
      \textbf{GPT-3.5}: Fear, \correct{Sadness}, Pain, Anger, Disquietment, \correct{Sympathy}\\
      \textbf{CLIP}: Anger, Fatigue, \wrong{Affection}, Sensitivity, \correct{Sadness}, \correct{Sympathy} \\
      % \textbf{LLaVA response}: Based on the visual cues in the image, the person in the red bounding box appears to be experiencing a mix of emotions. Most likely, they are feeling a combination of sadness, sympathy, and perhaps some fear or anxiety. It's important to note that the image may not capture the full range of the person's emotions, and the interpretation is based on the prominent emotions discernible in the visual cues provided.\\
      \textbf{LLaVA}: \correct{Sadness}, \correct{Sympathy}, Fear\\

      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{8. GT}: Happiness, Pleasure\\
      \textbf{NarraCap}: This person is an adult who is shaking hands at a board room. This person is engaging excitedly with others. This person is using a strong, businesslike handshake.\\
      \textbf{GPT-3.5}: Confidence, Engagement, \correct{Happiness}, \correct{Pleasure}, Excitement, Anticipation\\
      \textbf{CLIP}: \wrong{Suffering}, \wrong{Disconnection}, Sensitivity, Esteem, Confidence, Engagement\\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box is likely experiencing a mixture of emotions. They might be feeling happy, as they are smiling, and engaged in a handshake or greeting with the person in the blue shirt. They could also be feeling a sense of professionalism and respect, given that they are dressed in business attire, along with the other people in the image. However, the person may also be experiencing some nervousness, excitement, or anticipation, as they are making a handshake, which is often associated with formal events, job interviews, or networking opportunities. The woman's long hair might be an additional detail that contributes to the overall perception of her appearance, but it does not necessarily influence her emotions or the situation at hand.\\
      \textbf{LLaVA}: Excitement, Anticipation\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      \textbf{9. GT}: Affection, Engagement, Happiness, Pleasure\\
      \textbf{NarraCap}: This person is a baby who is grooming a dog at a vet clinic. This person is displaying affection with friends or loved ones. This person is gazing at someone, full of love.\\
    \textbf{GPT-3.5}: \correct{Affection}, \correct{Happiness}, Peace, \correct{Pleasure}, Esteem, Excitement
\\
    \textbf{CLIP}: \wrong{Sadness}, \correct{Engagement}, Peace, \correct{Happiness}, \correct{Pleasure}, \correct{Affection}\\
    % \textbf{LLaVA response}: The person in the red bounding box appears to be experiencing a range of emotions, including happiness, affection, and a sense of connection with the puppy. They are likely enjoying the moment as they hug the puppy and smell its fur. Additionally, the person may also feel surprise, as the interaction with the puppy might be unexpected or heartwarming, leading to feelings of joy and warmth. Sympathy and support for the puppy's wellbeing could also be present, as the person engages with the dog in a loving and caring manner.\\
      \textbf{LLaVA}: \correct{Happiness}, \correct{Affection}, Surprise, Sympathy\\
      \hline
    \end{tabular} \\
  \end{tabular}
  \vspace{-2mm}
  \caption{Qualitative results of EMOTIC images, ground truth (GT) labels, captions and inferred labels.}
    \label{tab:images}
  \vspace{-4mm}
\end{table*}


==> tables/qualitative2.tex <==
\begin{table*}[htbp]
\small
  \centering
  \caption{Qualitative results}
  \label{tab:images}

  \begin{tabular}{p{1cm}|p{4.5cm}|p{4.5cm}|p{4.5cm}|}
    & \includegraphics[width=0.25\textwidth]{imgs/COCO_val2014_000000070426_0.jpg} &
    \includegraphics[width=0.25\textwidth]{imgs/COCO_val2014_000000084694_0.jpg} &
    \includegraphics[width=0.25\textwidth]{imgs/COCO_train2014_000000353009_0.jpg} \\
    
      \hline
      \textbf{GT} & happiness, peace, pleasure
      & anticipation, confidence, engagement, excitement, happiness, peace 
      & anticipation, confidence, esteem
      \\
      \hline
      \textbf{Narra-Cap} & This person is an older woman who is surfing water at a beach. She has saggy posture, bent neck. She has chin dipping to the chest, adopting a slumped posture. She is participating in relaxing activities.
      &
      This person is an older man who is tasting wine at a wine cellar. He has hands laying in the lap. He has fingers loosely clasped in one's lap. He is unbuttoning the top button of a shirt.
      &
      This person is an older man who is doing a tennis swing at a rec center. He has leg muscles tightening. He is clasping one's forearms, elbows pressed to the sides. He is using the body to nudge, push, or block (line jumpers).
      \\
      \hline
      \textbf{GPT-3} & confidence, engagement, happiness, peace, pleasure, sympathy
      &
      confidence, engagement, happiness, pleasure, esteem, anticipation
      &
      confidence, engagement, happiness, pleasure, excitement, anticipation
      \\
      \hline
      \textbf{CLIP} & happiness, sympathy, embarrassment, peace, confidence, esteem
      &
      disquietment, peace, sadness, sympathy, doubt/confusion, surprise
      &
      doubt/confusion, esteem, confidence, fatigue, sensitivity, suffering
      \\
      
    \hline\hline
    
    & \includegraphics[width=0.25\textwidth]{imgs/frame_4rauu3fxrxpl6t8w_0.jpg} &
    \includegraphics[width=0.25\textwidth]{imgs/egnw6lbc92pja8wkok_1.jpg} &
    \includegraphics[width=0.25\textwidth]{imgs/fn3o5z0u9vxkzs2giz_0.jpg} \\
    \hline
    
      \textbf{GT} & fatigue, peace
      &
      disapproval, disquietment, fear, sadness, suffering
      &
      affection, anger, annoyance, disapproval, disquietment, doubt/confusion, fear, sadness
      \\
      \hline
      \textbf{Narra-Cap} & This person is an older man who is sleeping at a library. He is sleeping. He is curling up to take up less space. He is falling asleep in odd places at odd times.
      &
      This person is an older woman who is huddling at a city bus. She is covering oneself (closing a jacket). She is squeezing the eyes shut, refusing to look. She is crying, wailing, begging for help.
      &
      This person is an older woman who is having a pillow fight at a run-down apartment. She is placing trembling fingertips against one's open mouth. She is squeezing the eyes shut, refusing to look. She is tossing and turning in bed, an inability to sleep.
      
      \\
      \hline
    \textbf{GPT-3} & fear, fatigue, disquietment, embarrassment, disconnection, sadness
    &
    fear, sadness, embarrassment, disquietment, anger, sympathy
    &
    Fear, annoyance, fatigue, embarrassment, sadness, sympathy
    \\
    \hline
    \textbf{CLIP} & sympathy, engagement, suffering, disquietment, disconnection, fatigue
    &
    engagement, esteem, fear, sensitivity, sadness, sympathy
    &
    aversion, sympathy, sensitivity, disquietment, anger, fatigue
    \\
      \hline
  \end{tabular}
  
\end{table*}


==> tables/qualitative_failure.tex <==
\begin{table*}[t]
\vspace{-15mm}
\tiny
  \centering
  \begin{tabular}{ccc}
   \includegraphics[width=0.3\textwidth]{latex/imgs/b3fmbjeeaz873xzcpu_1.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/ddkop7rtr67verjpfd_0.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/COCO_train2014_000000353009_0.jpg} \\
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      % \textbf{1. GT}: Affection, Doubt/Confusion, Sympathy\\
      \textbf{1}: This person is an adult who is \wrong{acting in a play} at a therapist office. This person is \wrong{not engaging in conversation.}\\
    % \textbf{GPT-3.5}: Aversion, Disapproval, Fear, Annoyance, Disquietment, Embarrassment\\
    % \textbf{CLIP}: Disconnection, Disquietment, Esteem, Sensitivity, Anger, Engagement\\
    % \textbf{LLaVA response}:The person in the red bounding box appears to be experiencing a range of emotions, including sadness, sympathy, and possibly fear or concern. They may be feeling sad or empathetic towards the other woman who has her arms folded and is seemingly upset or frustrated. The presence of a couch and remote in the image suggests that they are in a living room, adding to the intimate and personal nature of their interaction. The combination of expressions and body language, along with the presence of a cell phone, indicates that the two women may be engaged in a deep conversation or discussing a difficult topic.\\
    % \textbf{LLaVA}: Sadness, Sympathy, Fear\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      % \textbf{2. GT}: Anger, Annoyance, Confidence, Engagement, Excitement, Pain, Suffering\\
      \textbf{2}: This person is a \wrong{baby} who is punching a person (boxing) at a sporting event stands. This person is \wrong{chewing on a knuckle}. This person is \wrong{propping the head up with fist}. \wrong{This person is responding with anger by punching.}\\
      % \textbf{GPT-3.5}: Anger, Fear, Annoyance, Disquietment, Embarrassment, Excitement\\
      % \textbf{CLIP}: Suffering, Disapproval, Annoyance, Embarrassment, Sympathy, Anger\\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mix of emotions. The most likely labels they are feeling would include excitement, anticipation, and happiness, as they are engaged in a boxing match and possibly celebrating a victory. They might also be feeling a sense of annoyance or discomfort due to the physical contact with the other boxer. Additionally, they could be experiencing sadness or sympathy for the other boxer, as the fight is competitive, and the emotions of both fighters are likely to be complex. Overall, the range of emotions experienced during a boxing match can vary, and the person in the red bounding box is likely experiencing a combination of these emotions during the fight.\\
      % \textbf{LLaVA}: Excitement, Anticipation, Happiness, Annoyance, Sadness, Sympathy\\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline 
    % \textbf{3. GT}: Anticipation, Confidence, Esteem\\
      \textbf{3}:
      This person is an \wrong{elderly} person who is doing a tennis swing at a rec center. This person has leg muscles tightening. This person is using the body to nudge, push, or block.\\
      % \textbf{GPT-3.5}: Confidence, Engagement, Happiness, Pleasure, Excitement, Anticipation\\
      % \textbf{CLIP}: Doubt/Confusion, Esteem, Confidence, Fatigue, Sensitivity, Suffering\\
      % \textbf{LLaVA response}: The person in the red bounding box is likely experiencing a mixture of emotions, including anguish, fear, and sadness, as they are caught in a difficult situation. They may also feel sympathy, as they are seen playing tennis in the black and white photo, possibly with others. The image shows the person is attempting to hit the tennis ball with their racquet, which indicates they are engaged in the game. The fact that the person is in a red box suggests they are the central focus of the scene, and their emotions might be linked to their performance or the outcome of the game.\\
      % \textbf{LLaVA}: Fear, Sadness, Sympathy\\
      \hline
    \end{tabular} \\
    % \includegraphics[width=0.3\textwidth]{latex/imgs/f36j0deu657obta0ln_0.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/frame_hgnlox6nq0yw9qbg_1.jpg} &
    \includegraphics[width=0.3\textwidth]{latex/imgs/egnw6lbc92pja8wkok_1.jpg}  &
    \includegraphics[width=0.3\textwidth]{latex/imgs/fn3o5z0u9vxkzs2giz_0.jpg}  \\
    
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      % \textbf{4. GT}: Aversion, Disquietment, Fear, Sadness, Sensitivity, Suffering\\
      \textbf{4}: This person is an adult who is longboarding at a skate park. This person has fingers loosely clasped in one's lap. This person has raised, prominent cheekbones from smiling. This person is \wrong{rubbing one's hands on pant legs.}\\
      
      % This person is an adult who is \wrong{twiddling fingers} at a \wrong{attic}. This person has lips pulling back, baring the teeth. This person has \wrong{skin stretched into a snarl}. This person is \wrong{placing fingertips against one's open mouth}.\\

      
    % \textbf{GPT-3.5}: Fear, Anger, Disapproval, Aversion, Annoyance, Disquietment\\
    % \textbf{CLIP}: Sensitivity, Anger, Suffering, Doubt/Confusion, Disconnection, Fear\\
    % \textbf{LLaVA response}: Based on the image, the person in the red bounding box is most likely experiencing a mixture of fear, surprise, and disgust. The hand with long, sharp claws is reaching towards the person's face, which could provoke feelings of unease and threat. The close-up of the face also enhances the sense of immediacy and intensity of the emotions experienced by the person in the box. It is important to note that the image is open to interpretation, and other viewers may perceive different emotions or nuances in the scene \\
      % \textbf{LLaVA}: Fear, Surprise \\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      % \textbf{5. GT}: Disapproval, Disquietment, Fear, Sadness, Suffering\\
      \textbf{5}: This person is an \wrong{elderly} person who is \wrong{huddling} at a \wrong{city bus}. This person is crying, wailing, begging for help. This person is squeezing the eyes shut, refusing to look.\\
      % \textbf{GPT-3.5}: Fear, Pain, Anger, Sadness, Embarrassment, Sympathy\\
      % \textbf{CLIP}: Engagement, Esteem, Fear, Sensitivity, Sadness, Sympathy \\
      % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mixture of emotions, including sadness, distress, and vulnerability. With the group of people around her, it seems she is seeking comfort or support from others. Her head is covered, which might add to her feelings of distress or sadness. While some of the other people in the scene may also be experiencing hardships, the person in the red bounding box is the main focus, and her emotions are more prominently displayed. It is important to offer help and support to people in such situations to alleviate their pain and assist them in coping with their emotional turmoil\\
      % \textbf{LLaVA}: Sadness, Pain \\
      \hline
    \end{tabular} &
    \begin{tabular}{|p{0.3\textwidth}|}
      \hline
      % \textbf{6. GT}: Affection, Anger, Annoyance, Disapproval, Disquietment, Doubt/Confusion, Fear, Sadness\\
      \textbf{6}: This person is an adult who is having a \wrong{pillow fight} at a run-down apartment. This person is tossing and turning in bed, an inability to sleep.\\
    % \textbf{GPT-3.5}: Fear, Annoyance, Fatigue, Embarrassment, Excitement, Sadness\\
    % \textbf{CLIP}: Aversion, Sympathy, Sensitivity, Disquietment, Anger, Fatigue\\
    % \textbf{LLaVA response}: Based on the image of the woman with her hands over her face and the visual labels provided, it is likely that she is experiencing a combination of emotions, including sadness, fear, and possibly some confusion or discomfort. The scene might depict feelings of being overwhelmed, anxious or even experiencing a nightmare, given the visual context of the bed and the white pillow. It is important to note that emotions can be complex, and different people may experience different emotions or react differently to the same situation \\
      % \textbf{LLaVA}: Sadness, Fear \\
      \hline
    \end{tabular} \\
    % \includegraphics[width=0.3\textwidth]{latex/imgs/frame_hgnlox6nq0yw9qbg_1.jpg} &
    % \includegraphics[width=0.3\textwidth]{latex/imgs/sun_aiuphnodytonkden_1.jpg}  &
    % \includegraphics[width=0.3\textwidth]{latex/imgs/sun_avyraobmgdwerddj_0.jpg}  \\
    
    % \begin{tabular}{|p{0.3\textwidth}|}
    %   \hline
    %     % \textbf{7. GT}: Anger, Anticipation, Aversion, Engagement, Excitement, Happiness, Pleasure, Sympathy\\
    %   \textbf{7}:  This person is an adult who is longboarding at a skate park. This person has fingers loosely clasped in one's lap. This person has raised, prominent cheekbones from smiling. This person is \wrong{rubbing one's hands on pant legs.}\\
    % % \textbf{GPT-3.5}: Confidence, Engagement, Happiness, Peace, Pleasure, Esteem\\
    % % \textbf{CLIP}: Sadness, Surprise, Pain, Esteem, Excitement, Happiness \\
    % % \textbf{LLaVA response}: Based on the image, the person in the red bounding box is likely experiencing a mix of emotions. These may include happiness, as they are smiling, as well as a sense of belonging or camaraderie, since they are surrounded by four friends who are also holding skateboards. They might also feel excitement or anticipation, given their engagement in the activity of skateboarding and possibly waiting to perform tricks or enjoy the day ahead. While it is not possible to definitively confirm all six emotions, these are some plausible feelings the person in the red bounding box could be experiencing based on the visual cues provided.\\
    %   % \textbf{LLaVA}: Happiness, Excitement, Anticipation, Engagement\\
    %   \hline
    % \end{tabular} &
    % \begin{tabular}{|p{0.3\textwidth}|}
    %   \hline
    %   % \textbf{8. GT}: Disconnection, Engagement, Peace, Pleasure\\
    %   \textbf{8}: This person is a \wrong{baby} who is swinging at a \wrong{tree house}. This person is slouching in a chair \wrong{with one's arms dangling}.\\
    %   % \textbf{GPT-3.5}: Fear, Embarrassment, Annoyance, Fatigue, Disquietment, Sadness\\
    %   % \textbf{CLIP}: Sensitivity, Sympathy, Sadness, Excitement, Pain, Fear\\
    %   % \textbf{LLaVA response}: Based on the image, the person in the red bounding box appears to be experiencing a mix of emotions. The most likely labels they are feeling would include happiness, as they are on a swing at a park, enjoying the experience. Additionally, some sadness or disappointment may be present since they are described as missing their family and being in pain. The person may also be experiencing anticipation and excitement, as they are looking forward to coming home. Furthermore, the presence of the large purple ball and bench may indicate a sense of curiosity or interest in the surroundings.\\
    %   % \textbf{LLaVA}: Happiness, Sadness, Disappointment, Pain, Anticipation, Excitement\\
    %   \hline
    % \end{tabular} &
    % \begin{tabular}{|p{0.3\textwidth}|}
    %   \hline
    %   % \textbf{9. GT}: Confidence, Disconnection, Engagement, Happiness, Sympathy\\
    %   \textbf{9}: This person is an elderly person who is \wrong{conducting an auction} at a \wrong{university lecture hall}. This person is clasping the hands in front of the groin or other sensitive area.\\
    % % \textbf{GPT-3.5}: Fear, Embarrassment, Disquietment, Annoyance, Doubt/Confusion, Sadness\\
    % % \textbf{CLIP}: Sympathy, Sensitivity, Esteem, Disapproval, Embarrassment, Surprise\\
    % % \textbf{LLaVA response}: Given the image, the person in the red bounding box might be experiencing a mix of emotions. Six possible labels that the person could be feeling include happiness, excitement, anticipation, surprise, admiration, and sympathy. For instance, the person might be happy to attend the meeting, excited about a forthcoming event or discussion, and anticipating a positive outcome. They could also experience surprise at an unexpected development or revelation, feel admiration for a speaker or colleague, and empathize with others' emotions. However, without knowing the specific context, it is difficult to pinpoint the exact emotions the person in the red bounding box is experiencing.\\
    %   % \textbf{LLaVA}: Happiness, Excitement, Anticipation, Surprise, Sympathy\\
    %   \hline
    % \end{tabular} \\
  \end{tabular}
  \vspace{-2mm}
    \caption{Failure examples of narrative captions.}
  \label{tab:fail}
  \vspace{-4mm}
\end{table*}






==> tables/table2_pdf.tex <==
\begin{figure*}[t]
% \vspace{-15mm}
\centering
\includegraphics[width=1\linewidth]{imgs/fig4_acii.pdf}
%\framebox(500,300){}
%\framebox[\textwidth]{\rule{0pt}{140pt}}
\vspace{-7mm}
\caption{Failure examples of narrative captions.}
  \label{tab:fail}
\vspace{-4mm}
\end{figure*}
% }]

